Strictification of weakly stable type-theoretic structures using generic contexts

We present a new strictification method for type-theoretic structures that are only weakly stable under substitution. Given weakly stable structures over some model of type theory, we construct equivalent strictly stable structures by evaluating the weakly stable structures at generic contexts. These generic contexts are specified using the categorical notion of familial representability. This generalizes the local universes method of Lumsdaine and Warren. We show that generic contexts can also be constructed in any category with families which is freely generated by collections of types and terms, without any definitional equality. This relies on the fact that they support first-order unification. These free models can only be equipped with weak type-theoretic structures, whose computation rules are given by typal equalities. Our main result is that any model of type theory with weakly stable weak type-theoretic structures admits an equivalent model with strictly stable weak type-theoretic structures.

==> macros.tex <==
%%% General macros

% Abbreviations.
\makeatletter
\newcommand{\DeclareAbbrevation}[2]{\newcommand{#1}{\@ifnextchar{.}{#2}{#2.\@\xspace}}}
\makeatother

\DeclareAbbrevation{\ie}{i.e}
\DeclareAbbrevation{\eg}{e.g}
\DeclareAbbrevation{\cf}{cf}
\DeclareAbbrevation{\resp}{resp}
\DeclareAbbrevation{\etal}{et al}
\DeclareAbbrevation{\ibid}{ibid}
\DeclareAbbrevation{\ca}{ca}
\DeclareAbbrevation{\vs}{vs}
\DeclareAbbrevation{\etc}{etc}

% End of definitions
% \DeclareRobustCommand{\defiEnd}{%
%   \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
%   \quad\hbox{$\lrcorner$}%
% }

% Lowercase mathcal
\DeclareFontFamily{U}{mathc}{}
\DeclareFontShape{U}{mathc}{m}{it}%
{<->s*[1.03] mathc10}{}
\DeclareMathAlphabet{\mathcal}{U}{mathc}{m}{it}

% Japanese letters (for the Yoneda embedding)
\DeclareFontFamily{U}{min}{}
\DeclareFontShape{U}{min}{m}{n}{<-> udmj30}{}

% Emphasis
\newcommand{\defemph}[1]{\textbf{#1}}
\newcommand{\deemph}[1]{\textcolor{gray}{#1}}

% Double langle/rangle
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother

% Arrows
\newcommand{\uda}{\updownarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\hra}{\hookrightarrow}
\newcommand{\rat}{\rightarrowtail}
\newcommand{\ratri}{\rightarrowtriangle}
\newcommand{\thra}{\twoheadrightarrow}
\newcommand{\thla}{\twoheadleftarrow}
\newcommand{\rsqa}{\rightsquigarrow}
\newcommand{\tfibra}{\stackrel{\sim}{\smash{\thra}\rule{0pt}{0.4ex}}}

% Brackets
\newcommand{\parens}[1]{{\left( #1 \right)}}
\newcommand{\abs}[1]{{\left| #1 \right|}}
\newcommand{\sem}[1]{{\llbracket #1 \rrbracket}}
\newcommand{\lens}[1]{{\llparenthesis #1 \rrparenthesis}}
\newcommand{\trunc}[1]{{\parallel #1 \parallel}}
\newcommand{\angles}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\uquote}[1]{{\ulcorner #1 \urcorner}}
\newcommand{\dquote}[1]{{\dlcorner #1 \drcorner}}

%%% Short names

% Short names for models (mathbb)
\newcommand{\MA}{\mathbb{A}}
\newcommand{\MB}{\mathbb{B}}
\newcommand{\MC}{\mathbb{C}}
\newcommand{\MD}{\mathbb{D}}
\newcommand{\ME}{\mathbb{E}}
\newcommand{\MF}{\mathbb{F}}
\newcommand{\MG}{\mathbb{G}}
\newcommand{\MH}{\mathbb{H}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MJ}{\mathbb{J}}
\newcommand{\MK}{\mathbb{K}}
\newcommand{\ML}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\MN}{\mathbb{N}}
\newcommand{\MO}{\mathbb{O}}
\newcommand{\MP}{\mathbb{P}}
\newcommand{\MQ}{\mathbb{Q}}
\newcommand{\MR}{\mathbb{R}}
\newcommand{\MS}{\mathbb{S}}
\newcommand{\MT}{\mathbb{T}}
\newcommand{\MU}{\mathbb{U}}
\newcommand{\MV}{\mathbb{V}}
\newcommand{\MW}{\mathbb{W}}
\newcommand{\MX}{\mathbb{X}}
\newcommand{\MY}{\mathbb{Y}}
\newcommand{\MZ}{\mathbb{Z}}


\newcommand{\Ma}{\mathbb{a}}
\newcommand{\Mb}{\mathbb{b}}
\newcommand{\Mc}{\mathbb{c}}
\newcommand{\Md}{\mathbb{d}}
\newcommand{\Me}{\mathbb{e}}
\newcommand{\Mf}{\mathbb{f}}
\newcommand{\Mg}{\mathbb{g}}
\newcommand{\Mh}{\mathbb{h}}
\newcommand{\Mi}{\mathbb{i}}
\newcommand{\Mj}{\mathbb{j}}
\newcommand{\Mk}{\mathbb{k}}
\newcommand{\Ml}{\mathbb{l}}
\newcommand{\Mm}{\mathbb{m}}
\newcommand{\Mn}{\mathbb{n}}
\newcommand{\Mo}{\mathbb{o}}
\newcommand{\Mp}{\mathbb{p}}
\newcommand{\Mq}{\mathbb{q}}
\newcommand{\Mr}{\mathbb{r}}
\newcommand{\Ms}{\mathbb{s}}
\newcommand{\Mt}{\mathbb{t}}
\newcommand{\Mu}{\mathbb{u}}
\newcommand{\Mv}{\mathbb{v}}
\newcommand{\Mw}{\mathbb{w}}
\newcommand{\Mx}{\mathbb{x}}
\newcommand{\My}{\mathbb{y}}
\newcommand{\Mz}{\mathbb{z}}


% Short names for sets and internal things (mathrm / mathsf)
\newcommand{\SProp}{\mathrm{Prop}}
\newcommand{\SSet}{\mathrm{Set}}
\newcommand{\SCat}{\mathrm{Cat}}
\newcommand{\SCwf}{\mathrm{CwF}}

\newcommand{\cxl}{\mathsf{cxl}}
\newcommand{\dem}{\mathsf{dem}}

\newcommand{\SA}{\mathsf{A}}
\newcommand{\SB}{\mathsf{B}}
\newcommand{\SC}{\mathsf{C}}
\newcommand{\SD}{\mathsf{D}}
\newcommand{\SE}{\mathsf{E}}
\newcommand{\SF}{\mathsf{F}}
\newcommand{\SG}{\mathsf{G}}
\newcommand{\SH}{\mathsf{H}}
\newcommand{\SI}{\mathsf{I}}
\newcommand{\SJ}{\mathsf{J}}
\newcommand{\SK}{\mathsf{K}}
\newcommand{\SL}{\mathsf{L}}
\newcommand{\SM}{\mathsf{M}}
\newcommand{\SN}{\mathsf{N}}
\newcommand{\SO}{\mathsf{O}}
\newcommand{\SP}{\mathsf{P}}
\newcommand{\SQ}{\mathsf{Q}}
\newcommand{\SR}{\mathsf{R}}
\renewcommand{\SS}{\mathsf{S}}
\newcommand{\ST}{\mathsf{T}}
\newcommand{\SU}{\mathsf{U}}
\newcommand{\SV}{\mathsf{V}}
\newcommand{\SW}{\mathsf{W}}
\newcommand{\SX}{\mathsf{X}}
\newcommand{\SY}{\mathsf{Y}}
\newcommand{\SZ}{\mathsf{Z}}

\newcommand{\Sa}{\mathsf{a}}
\newcommand{\Sb}{\mathsf{b}}
\newcommand{\Sc}{\mathsf{c}}
\newcommand{\Sd}{\mathsf{d}}
\newcommand{\Se}{\mathsf{e}}
\newcommand{\Sf}{\mathsf{f}}
\newcommand{\Sh}{\mathsf{h}}
\newcommand{\Sg}{\mathsf{g}}
\newcommand{\Si}{\mathsf{i}}
\newcommand{\Sj}{\mathsf{j}}
\newcommand{\Sk}{\mathsf{k}}
\newcommand{\Sl}{\mathsf{l}}
\newcommand{\Sm}{\mathsf{m}}
\newcommand{\Sn}{\mathsf{n}}
\newcommand{\So}{\mathsf{o}}
\newcommand{\Sp}{\mathsf{p}}
\newcommand{\Sq}{\mathsf{q}}
\newcommand{\Sr}{\mathsf{r}}
\newcommand{\Ss}{\mathsf{s}}
\newcommand{\St}{\mathsf{t}}
\newcommand{\Su}{\mathsf{u}}
\newcommand{\Sv}{\mathsf{v}}
\newcommand{\Sw}{\mathsf{w}}
\newcommand{\Sx}{\mathsf{x}}
\newcommand{\Sy}{\mathsf{y}}
\newcommand{\Sz}{\mathsf{z}}

% Short names for categories (mathbf or mathcal)
\newcommand{\CSet}{\mathbf{Set}}
\newcommand{\CProp}{\mathbf{Prop}}
\newcommand{\CPsh}{\mathbf{Psh}}
\newcommand{\CCat}{\mathbf{Cat}}
\newcommand{\CCwf}{\mathbf{CwF}}
\newcommand{\CMod}{\mathbf{Mod}}

\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}

\newcommand{\BA}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\BC}{\mathbf{C}}
\newcommand{\BD}{\mathbf{D}}
\newcommand{\BE}{\mathbf{E}}
\newcommand{\BF}{\mathbf{F}}
\newcommand{\BG}{\mathbf{G}}
\newcommand{\BH}{\mathbf{H}}
\newcommand{\BI}{\mathbf{I}}
\newcommand{\BJ}{\mathbf{J}}
\newcommand{\BK}{\mathbf{K}}
\newcommand{\BL}{\mathbf{L}}
\newcommand{\BM}{\mathbf{M}}
\newcommand{\BN}{\mathbf{N}}
\newcommand{\BO}{\mathbf{O}}
\newcommand{\BP}{\mathbf{P}}
\newcommand{\BQ}{\mathbf{Q}}
\newcommand{\BR}{\mathbf{R}}
\newcommand{\BS}{\mathbf{S}}
\newcommand{\BT}{\mathbf{T}}
\newcommand{\BU}{\mathbf{U}}
\newcommand{\BV}{\mathbf{V}}
\newcommand{\BW}{\mathbf{W}}
\newcommand{\BX}{\mathbf{X}}
\newcommand{\BY}{\mathbf{Y}}
\newcommand{\BZ}{\mathbf{Z}}

% mathfrak letters
\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}

%%% Category theory

% Categorical structure
\newcommand{\Ob}{\mathsf{Ob}}
\newcommand{\Hom}{\mathsf{Hom}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\op}{\mathsf{op}}

% Colimits
\DeclareMathOperator*{\colim}{colim}

% Presheaf categories
\newcommand{\psh}[1]{\widehat{#1}}
% \newcommand{\yo}{\text{\usefont{U}{min}{m}{n}\symbol{'210}}}
\newcommand{\yo}{\mathbb{y}}

%%% Type theory

% Components of models of type theory
\newcommand{\type}{\mathsf{type}}
\newcommand{\Con}{\mathsf{Con}}
\newcommand{\Sub}{\mathsf{Sub}}
\newcommand{\Ty}{\mathsf{Ty}}
\newcommand{\ty}{\mathsf{ty}}
\newcommand{\Tm}{\mathsf{Tm}}
\newcommand{\tm}{\mathsf{tm}}
\newcommand{\Var}{\mathsf{Var}}
\newcommand{\var}{\mathsf{var}}

% Booleans
\newcommand{\Bool}{\mathbb{B}}
\newcommand{\BoolTy}{\mathbf{B}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\elimBool}{\mathsf{elim}_{\BoolTy}}

% Natural numbers
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\NatTy}{\mathbf{N}}
\newcommand{\zero}{\mathsf{zero}}
\newcommand{\suc}{\mathsf{suc}}
\newcommand{\elimNat}{\mathsf{elim}_{\NatTy}}

% Id-types
\newcommand{\Id}{\mathsf{Id}}
\newcommand{\J}{\mathsf{J}}
\newcommand{\Jbeta}{{\J\beta}}
\newcommand{\refl}{\mathsf{refl}}
\newcommand{\ap}{\mathsf{ap}}
\newcommand{\tr}{\mathsf{tr}}
\newcommand{\happly}{\mathsf{happly}}

% Eq-types
\newcommand{\Eq}{\mathsf{Eq}}

% Equivalences / hLevels
\newcommand{\Equiv}{\mathrm{Equiv}}
\newcommand{\isEquiv}{\mathrm{isEquiv}}
\newcommand{\isContr}{\mathrm{isContr}}
\newcommand{\isProp}{\mathrm{isProp}}
\newcommand{\isSet}{\mathrm{isSet}}
\newcommand{\isLinv}{\mathrm{isLInv}}
\newcommand{\isRinv}{\mathrm{isRInv}}

% Pi-types
\newcommand{\app}{\mathsf{app}}
\newcommand{\lam}{\mathsf{lam}}
\newcommand{\funext}{\mathsf{funext}}

% Sigma and Unit-types
\newcommand{\pair}{\mathsf{pair}}
\newcommand{\fst}{\mathsf{fst}}
\newcommand{\snd}{\mathsf{snd}}

\newcommand{\Unit}{\mathbf{1}}
\renewcommand{\tt}{\mathsf{tt}}

\newcommand{\Init}{\mathbf{0}}
\newcommand{\absurd}{\mathsf{absurd}}

% Quotients
\newcommand{\Quot}{\mathbf{Q}}
\newcommand{\quot}{\mathbf{q}}

% Universes
\newcommand{\UU}{\mathcal{U}}
\newcommand{\UV}{\mathcal{V}}

% Circled dollar symbol
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.1pt] (char) {#1};}}
\newcommand{\circleddollar}{\mathbin{\circled{\scalebox{0.7}{$\$$}}}}

% MTT Colors
\newcommand{\modcolor}[1]{\textcolor{orange!60!black}{#1}}
\newcommand{\natcolor}[1]{\textcolor{teal}{#1}}
\newcommand{\tickcolor}[1]{\textcolor{white!70!black}{#1}}

% Multimodal type theory

\newcommand{\modm}[1]{\{\modcolor{#1}\}} % Modality
\newcommand{\modt}[1]{\{\tickcolor{#1}\}} % Tick
\newcommand{\modtm}[2]{\{\tickcolor{#1} \colon\modcolor{#2}\}} % Tick and modality

\newcommand{\keyn}[1]{[\natcolor{#1}]} % (natural) transformation
\newcommand{\keytt}[2]{[\tickcolor{#1} / \tickcolor{#2}]} % tick -> tick
\newcommand{\keymm}[2]{[\modcolor{#1} / \modcolor{#2}]} % mod -> mod
\newcommand{\keyntt}[3]{[\natcolor{#1} \colon\tickcolor{#2} / \tickcolor{#3}]} % natural transformation : tick -> tick
\newcommand{\keynmm}[3]{[\natcolor{#1} \colon\modcolor{#2} / \modcolor{#3}]} % natural transformation : mod -> mod

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

